Proton structure at the LHC

A determination of Parton Distribution Functions (PDFs) from a global fit to a dataset including measurements from the LHC has been performed. The determinations have been carried out according to the NNPDF methodology, leading to a fit minimising parametrisation bias and with an accurate account of PDF uncertainty. In this thesis the importance of QCD measurements at the LHC to PDF extraction are discussed, and we summarise some of the technical difficulties in their inclusion into PDF fits. A number of methods are presented that permit the efficient inclusion of these observables into PDF determinations. Firstly a Bayesian reweighting procedure taking advantage of the Monte Carlo representation of PDF uncertainties in NNPDF sets is discussed, which is demonstrated by a study of the impact of early W production asymmetry measurements from ATLAS, CMS and LHCb upon an earlier PDF set. A package for the fast computation of observables in an automated NLO framework is presented, providing an interface between Monte Carlo event generators and NLO interpolation tools. Finally, a method of combining PDF evolution with interpolating codes for hadronic observable computation is described. This method largely overcomes the computational difficulties in performing fast perturbative QCD predictions for collider observables. The method has been applied to the determination of PDFs from a global dataset including vector boson production data from LHCb, ATLAS and CMS along with inclusive jet data from ATLAS. Finally, the method of closure testing is introduced, and the method is applied to the study of the NNPDF methodology. A number of improvements are found in the minimisation and stopping procedures, which are adopted for the development of the next NNPDF release, NNPDF3.0.

==> 6-LHCimpact/tab-chi2res-aut-covexp.tex <==
Total  &   1.145&   1.162 &    1.101 &    1.139 &    1.105 &    1.139 &    1.101 &    1.142 &    0.971 &    0.993 \\  
 \hline 
NMC-pd              & $          0.97      $ & $          0.93      $  &  $          0.95      $  &  $          0.95      $  &  $         0.93      $ &  $         0.93      $ &  $          0.93      $  &  $          0.94      $  &  $  \lc     5.33 \rc  $  &  $  \lc     5.13 \rc  $  \\  
NMC                 & $          1.68      $ & $          1.58      $  &  $          1.61      $  &  $          1.59      $  &  $         1.62      $ &  $         1.57      $ &  $          1.59      $  &  $          1.56      $  &  $  \lc     1.89 \rc  $  &  $  \lc     1.83 \rc  $  \\  
SLAC                & $          1.34      $ & $          1.04      $  &  $          1.24      $  &  $          1.00      $  &  $         1.27      $ &  $         1.01      $ &  $          1.28      $  &  $          1.04      $  &  $  \lc     1.72 \rc  $  &  $  \lc     1.41 \rc  $  \\  
BCDMS               & $          1.21      $ & $          1.29      $  &  $          1.20      $  &  $          1.28      $  &  $         1.20      $ &  $         1.28      $ &  $          1.20      $  &  $          1.28      $  &  $  \lc     1.85 \rc  $  &  $  \lc     2.15 \rc  $  \\  
CHORUS              & $          1.10      $ & $          1.08      $  &  $          1.10      $  &  $          1.07      $  &  $         1.10      $ &  $         1.06      $ &  $          1.09      $  &  $          1.07      $  &  $  \lc     1.73 \rc  $  &  $  \lc     1.70 \rc  $  \\  
NTVDMN              & $          0.70      $ & $          0.50      $  &  $          0.43      $  &  $          0.56      $  &  $         0.42      $ &  $         0.51      $ &  $          0.42      $  &  $          0.48      $  &  $  \lc    26.69 \rc  $  &  $  \lc    21.13 \rc  $  \\  
 \hline
HERAI-AV            & $          1.04      $ & $          1.04      $  &  $          1.00      $  &  $          1.01      $  &  $         1.00      $ &  $         1.02      $ &  $          1.01      $  &  $          1.03      $  &  $          0.97      $  &  $          0.99      $  \\  
FLH108              & $          1.34      $ & $          1.23      $  &  $          1.29      $  &  $          1.20      $  &  $         1.29      $ &  $         1.20      $ &  $          1.29      $  &  $          1.21      $  &  $          1.35      $  &  $          1.25      $  \\  
ZEUS-H2             & $          1.21      $ & $          1.21      $  &  $          1.20      $  &  $          1.22      $  &  $         1.20      $ &  $         1.22      $ &  $          1.20      $  &  $          1.22      $  &  $          1.29      $  &  $          1.32      $  \\  
ZEUS $F_2^c$        & $          0.75      $ & $          0.81      $  &  $          0.82      $  &  $          0.90      $  &  $         0.80      $ &  $         0.90      $ &  $          0.81      $  &  $          0.86      $  &  $          0.71      $  &  $          0.77      $  \\  
H1 $F_2^c$          & $          1.50      $ & $          1.44      $  &  $          1.59      $  &  $          1.53      $  &  $         1.57      $ &  $         1.52      $ &  $          1.58      $  &  $          1.49      $  &  $          1.33      $  &  $          1.30      $  \\  
 \hline
DYE605              & $          0.94      $ & $          1.08      $  &  $          0.86      $  &  $          1.04      $  &  $         0.88      $ &  $         1.04      $ &  $          0.85      $  &  $          1.06      $  &  $  \lc     3.58 \rc  $  &  $  \lc     1.02 \rc  $  \\  
DYE886              & $          1.42      $ & $          1.69      $  &  $          1.27      $  &  $          1.58      $  &  $         1.27      $ &  $         1.55      $ &  $          1.24      $  &  $          1.55      $  &  $  \lc     5.65 \rc  $  &  $  \lc     5.14 \rc  $  \\  
 \hline
CDF $W$ asy         & $          1.88      $ & $          1.63      $  &  $          1.57      $  &  $          1.64      $  &  $         1.57      $ &  $         1.72      $ &  $          1.45      $  &  $          1.67      $  &  $          1.05      $  &  $          1.21      $  \\  
CDF $Z$ rap         & $          1.77      $ & $          2.38      $  &  $          1.80      $  &  $          2.03      $  &  $         1.77      $ &  $         2.17      $ &  $          1.76      $  &  $          2.13      $  &  $          1.32      $  &  $          1.37      $  \\  
D0 $Z$ rap          & $          0.57      $ & $          0.67      $  &  $          0.56      $  &  $          0.61      $  &  $         0.57      $ &  $         0.63      $ &  $          0.57      $  &  $          0.63      $  &  $          0.56      $  &  $          0.58      $  \\  
ATLAS $W,Z$         & $  \lc     1.57 \rc  $ & $  \lc     2.21 \rc  $  &  $          1.26      $  &  $          1.43      $  &  $         1.31      $ &  $         1.65      $ &  $  \lc     1.37 \rc  $  &  $  \lc     1.94 \rc  $  &  $          1.02      $  &  $          1.05      $  \\  
CMS $W$ el asy      & $  \lc     2.02 \rc  $ & $  \lc     1.27 \rc  $  &  $          0.82      $  &  $          0.81      $  &  $         1.09      $ &  $         0.99      $ &  $  \lc     1.32 \rc  $  &  $  \lc     1.20 \rc  $  &  $          0.87      $  &  $          0.85      $  \\  
LHCb $W$            & $  \lc     0.89 \rc  $ & $  \lc     1.13 \rc  $  &  $          0.67      $  &  $          0.83      $  &  $         0.77      $ &  $         0.98      $ &  $  \lc     0.76 \rc  $  &  $  \lc     1.03 \rc  $  &  $          0.74      $  &  $          0.72      $  \\  
 \hline
CDF RII $k_T$       & $          0.68      $ & $          0.65      $  &  $          0.60      $  &  $          0.68      $  &  $         0.61      $ &  $         0.67      $ &  $          0.60      $  &  $          0.67      $  &  $          0.60      $  &  $          0.59      $  \\  
D0 RII cone         & $          0.90      $ & $          0.98      $  &  $          0.84      $  &  $          0.94      $  &  $         0.84      $ &  $         0.93      $ &  $          0.84      $  &  $          0.94      $  &  $          0.85      $  &  $          0.92      $  \\  
ATLAS jets          & $  \lc     1.06 \rc  $ & $  \lc     0.95 \rc  $  &  $          1.00      $  &  $          0.94      $  &  $         1.00      $ &  $         0.92      $ &  $  \lc     1.01 \rc  $  &  $  \lc     0.94 \rc  $  &  $          0.98      $  &  $          0.93      $  \\  

